CRC-Aided Learned Ensembles of Belief-Propagation Polar Decoders

Polar codes have promising error-correction capabilities. Yet, decoding polar codes is often challenging, particularly with large blocks, with recently proposed decoders based on list-decoding or neural-decoding. The former applies multiple decoders or the same decoder multiple times with some redundancy, while the latter family utilizes emerging deep learning schemes to learn to decode from data. In this work we introduce a novel polar decoder that combines the list-decoding with neural-decoding, by forming an ensemble of multiple weighted belief-propagation (WBP) decoders, each trained to decode different data. We employ the cyclic-redundancy check (CRC) code as a proxy for combining the ensemble decoders and selecting the most-likely decoded word after inference, while facilitating real-time decoding. We evaluate our scheme over a wide range of polar codes lengths, empirically showing that gains of around 0.25dB in frame-error rate could be achieved. Moreover, we provide complexity and latency analysis, showing that the number of operations required approaches that of a single BP decoder at high signal-to-noise ratios.

==> old/results_old.tex <==
\section{Numerical Evaluations}
\label{sec:numerical_evaluations}
\vspace{-0.1cm} 
In this section we numerically evaluate the proposed ensemble scheme over a number of scenarios to prove its gains. First, we present the simulation setup in Subsection \ref{subsec:simulation}. Then, we study different partitioning 
% Second, we describe the decoders compared in our experimental study, detailing the different architectures in Subsection~\ref{subsec:decoders}. 
Afterwards, the data partitioning done using the CRC information is described in Subsection~\ref{subsec:data}. Then, diversity measures and \ac{ber} results for short and long codes are shown in Subsection~\ref{subsec:diversity} and Subsection~\ref{subsec:results}, respectively. Lastly, we present the latency analysis simulation in Subsection~\ref{subsec:latency_results}.
%-----------------------------------
%	Simulation
%-----------------------------------
\vspace{-0.4cm}
\subsection{Simulation}
\label{subsec:simulation}
In the simulation\footnote{The source code used in our experiments is available at \href{https://github.com/tomerraviv95/polar-ensembles}{https://github.com/tomerraviv95/polar-ensembles}}, we simulate AWGN (Additive white Gaussian noise) channel to randomly generate the data. First, we train the ensemble with various SNRs values using the methods described in Subsection~{\ref{subsec:training}}. Hyper-parameters sweep is performed in order to achieve the best FER results.

%-----------------------------------
%	Decoders
%-----------------------------------
% \vspace{-0.4cm}
% \subsection{Decoders}
% \label{subsec:decoders}
% Here we describe the evaluated benchmark decoders. \textcolor{red}{[AG] we used only FF arch - consider removing???}

%-----------------------------------
%	Data
%-----------------------------------
\vspace{-0.4cm}
\subsection{Data Partitioning}
\label{subsec:data}
As described in Subsection~{\ref{subsec:training}}, each of the decoders $\mathcal{F}_i^{w(i)}$ in the ensemble should be trained on a different subset of the data $\mathcal{X}^{(i)}$. In order to map each word in the data-set to its corresponds subset a mapping rule is required. In this research we investigated 3 different rules:

Uniform partition:
\begin{equation} \label{eq:uniform_partition}
    \mathcal{X}^{(i)}=\{r:\frac{\alpha(i-1)}{2^P} \leq \sum_{j=1}^{P}{r_j \cdot 2^{P-j-1}} < \frac{\alpha i}{2^P} \}
\end{equation}

CRC bits sum:
\begin{equation} \label{eq:bits_sum}
    \mathcal{X}^{(i)}=\{r:\sum_{j=1}^{P}{r_j}=i \}
\end{equation}

CRC bits sum modulo:
\begin{equation} \label{eq:bits_sum_mod}
    \mathcal{X}^{(i)}=\{r:(\sum_{j=1}^{P}{r_j})mod \, \alpha=i\}
\end{equation}

Where $\mathcal{X}^{(i)} \subset \mathcal{R}, r \in \{0,1\}^P$ and $r \neq{\bold{0}}$ (Equation \ref{eq:crc_partition}). By generating random messages and passing them through the encoder, channel and $\mathcal{F}_0^I$ we analyze how balanced each subset $\mathcal{X}^{(i)}$ as seen in Figure \ref{fig:crc_histogram}. As can be seen, partition presented in Equation \ref{eq:uniform_partition} , \ref{eq:bits_sum_mod} resulted in most balanced set and also achieved better performance than the less balanced partition from Equation \ref{eq:bits_sum}. We note also that for different SNRs the CRC distribution is similar. The histograms in Figure \ref{fig:crc_histogram} were generated by passing $10^5$ randomly generated messages of Polar code $(64,32)$ through a channel with $SNR = 3 [dB]$ and then decoded by $\mathcal{F}_0^I$ which consist of 5 iterations, the partition is corresponds to number of decoders in the ensemble $\alpha=4$.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/crc_histogram.jpg}
    \caption{CRC distribution}
    \label{fig:crc_histogram}
\end{figure}


%-----------------------------------
%	Diversity
%-----------------------------------
\vspace{-0.4cm}
\subsection{Diversity}
\label{subsec:diversity}
Here we present the diversity analysis.
As described in Section \ref{sec:polar_ensembles}, the model designed to take advantage of the diversity of models, where each model trained on a specific range of CRC values. To analyze this effectiveness of the diversity, we generated a histogram that represent the difference between decoder performance and the CRC region that they were trained on. Each bin in the histogram represents the amount of correctly decoded words. Each color represents a WBP in the ensemble and each bin group represent the CRC values range that is the decision rule of by which we train the decoders. Each such range has one bin that does not have black bar above it, this bin represents the decoder of which we trained on this specific CRC range, and we address it the “designated decoder”.
The black bar above each bin is the number of words that the corresponds decoder successfully decoded while the designated decoder failed. For example, take $\alpha=4$ and CRC partition of Equation \ref{eq:bits_sum_mod}, then on the left plot in Figure \ref{fig:crc_diversity}, the $3^{rd}$ bin represent the amount of correctly decoded words with r corresponds to $(\sum_{j=1}^{P}{r_j})mod \, \alpha=2$, and each bar is corresponds to $\{\mathcal{F}_1^w^{(1)}, \mathcal{F}_1^w^{(2)}, \mathcal{F}_1^w^{(3)},\mathcal{F}_4^w^{(4)}\}$ by ascending order from left to right. The decoder which is trained on that CRC range is $\mathcal{F}_1^w^{(3)}$ thus the $3^{rd}$ bar on the $3^{rd}$ bin has no "black" region.
We can see that for each CRC region in the ensemble, the decoder that was trained on the corresponding CRC region didn't necessarily decode the most words, compared to the other decoders in the ensemble. It indicates that the training method failed to train the decoder to have optimal performance for the CRC region it was trained on. We infer that neither of the CRC partition we examined was able to divide the CRC values to different error patterns that the models could be trained on and create a mixture of experts ensemble.
However, we can observe that the proposed training method was able to train the models diversely, since there is a significant number of words that the designated decoder wasn't able to decode correctly and one of the other decoders in the ensemble decoded it correctly. As seen in Subsection~\ref{subsec:data} these both partitions also have balanced CRC value distribution, and this leads us to assume that as long the partitions are balanced, we can expect similar result. Also. this analysis lead us to using the ensemble in the decoded process as described in Subsection~\ref{subsec:decoding} by taking the successful decoder rather than the designated one.
Figure~\ref{fig:crc_diversity} generated by analyzing the simulation results for Polar code (64,32), ensemble model with $\alpha=4$ decoders and a batch of $10^4$ words that passed through the model.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/crc_diversity.jpg}
    \caption{CRC diversity}
    \label{fig:crc_diversity}
\end{figure}

%-----------------------------------
%	Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{Results}
\label{subsec:results}
The model was trained using the algorithm described in Subsection~\ref{subsec:training}, the data partition done according to uniform division Equation~\ref{eq:uniform_partition}, number of decoders $\alpha \in \{2,4,8\}$, WBP batch size=$200$, ensemble batch size=$500 \cdot \alpha$, training SNRs $\in \{1.25,2.255,3.25,4.25\}[dB]$, validation SNR=$2.75[dB]$, number of epochs=$200$, learning rate=$0.01$, adam optimizer. Each epoch contains different randomly generated messages that passed through the channel's simulation with SNR $\in$ training SNRs. For each epoch $e$ which holds $mod(e,5)=0$ the BER is calculated for each decoder using:
\begin{equation} \label{eq:ber}
    BER_i=\frac{1}{K}\sum_{v=1}^{K'}Pr(\mathcal{F}_i^{w(i)}(l) \neq u)
\end{equation}

Evaluation is done for BER and FER performance of the proposed algorithm using the simulation dectibed in Subsection~\ref{subsec:simulation}. The simulation estimates the BER and FER performance by generating input messages randomly and passing them in batches with size of 104 through the encoder, simulated channel, and the decoder. Counting the number of bit errors and frame (block) error until the number of frame errors is greater or equal to 500. Then, the simulation estimates the BER and FER by dividing the number of bit error and frame error counted respectively by the number of messages transmitted. 
It can be observed that as the number of decoders in the ensemble decreases the error ratio of the proposed algorithm, which indicates that our training method was able to train the models to be sufficiently diverse. This effect is also more noticeable as code length is increase, while on the shorter coder lengths $(256,128), (64,32)$ we see almost no performance gap between using 4 or 2 decoders in the ensemble, thus complexity can be decreased while maintaining the same performance using only 2 decoders.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/FER_BER_64_32.jpg}
    \caption{FER, BER (64,32)}
    \label{fig:FER_BER_64_32}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/FER_BER_256_128.jpg}
    \caption{FER, BER (256,128)}
    \label{fig:FER_BER_256_128}
\end{figure}

%-----------------------------------
%	Latency Analysis
%-----------------------------------
\vspace{-0.4cm}
\subsection{Latency Analysis}
\label{subsec:latency_results}
As described in Subsection~\ref{subsec:latency}, the complexity of the model can be estimated using Equation~\ref{eq:flops}, and from it to derive the latency of the applied system. The Figures~\ref{fig:flops_64_32}-\ref{fig:flops_1024_512} where evaluated by taking the FER results of $\mathcal{F}_0^I$ for each code length and using it in Equation~\ref{eq:flops}. We plot also the lower bound which is the flops of $\mathcal{F}_0^I$ (in the case the ensemble is not being used). The upper line is a reference and is represent the flops of a equivalence WBP in terms of total parameters to the decoder.
As can be seen in Figure~\ref{fig:flops_64_32}, in case of shorter code length, complexity wise the ensemble is always better compared to similar number of parameters WBP decoder. On longer code length Figures~\ref{fig:flops_256_128}-\ref{fig:flops_1024_512} we see that there is a SNR threshold in which the ensemble become less complex than the comparable WBP. This threshold is increasing with the code length and it’s a direct result from that the FER is higher on longer codes when the SNR is low, as can be seen in Subsection~\ref{subsec:results}. In all cases we see convergence to single BP complexity as SNR increase, which means that the $Latency_{excess}$ is minimised while keeping the advantages of the ensemble.
It important to note that latency wise, our model can be parallelized opposed to higher iteration amount WBP model, as each WBP in the ensemble is independent with the others and reduce even lower the $Latency_{excess}$. It is also possible to run the ensemble in parallel to $\mathcal{F}_0^I$ and by decoding the words by all of the WBPs at once and taking only the correctly decoded word. This implementation achieves the latency of single BP and reducing the $Latency_{excess}$ to 0, while preserving the advantages of higher complexity WBPs in the cost of higher computational power.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/flops_64_32.jpg}
    \caption{Flops (64,32) , \alpha \in \{4,8\}}
    \label{fig:flops_64_32}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/flops_256_128.jpg}
    \caption{Flops (256,128), \alpha \in \{4,8\}}
    \label{fig:flops_256_128}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/flops_1024_512.jpg}
    \caption{Flops (1024,512), \alpha \in \{4,8\}}
    \label{fig:flops_1024_512}
\end{figure}
